Curriculum Script Distillation for Multilingual Visual Question Answering

Pre-trained models with dual and cross encoders have shown remarkable success in propelling the landscape of several tasks in vision and language in Visual Question Answering (VQA). However, since they are limited by the requirements of gold annotated data, most of these advancements do not see the light of day in other languages beyond English. We aim to address this problem by introducing a curriculum based on the source and target language translations to finetune the pre-trained models for the downstream task. Experimental results demonstrate that script plays a vital role in the performance of these models. Specifically, we show that target languages that share the same script perform better (~6%) than other languages and mixed-script code-switched languages perform better than their counterparts (~5-12%).

==> tables/data.tex <==
%%%%%%%%%%%% start
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[tbh]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{llllll}
\hline
\textbf{Task} & \textbf{Src} & \textbf{Citation} & \textbf{Languages} & \textbf{Gold/Silver} & \textbf{Parallel?} \\ \hline
Image Captioning, & IAPR & \cite{grubinger2006iapr} & de, es & Gold & Yes \\
Retreival & Pascal Sentences & \cite{DBLP:conf/emnlp/FunakiN15} & ja & Gold & Yes \\
 & Flickr8k & \cite{DBLP:conf/mir/LiLDL16} & zh & Gold Test & Yes \\
 & Flickr30k & \cite{DBLP:conf/mm/LanLD17} & zh & Gold Test & Yes \\
 &  & \cite{nakayama-etal-2020-visually} & ja & Gold & Yes \\
 &  & \cite{DBLP:conf/acl/ElliottFSS16} & de, fr, cs & Gold & Yes \\
 & Multi30k & \cite{DBLP:conf/lrec/LalaS18} & de, fr & Silver + Gold & No \\
 & MSCOCO & \cite{DBLP:journals/tmm/LiXWLJYX19} & zh & Gold test & Yes \\
 &  & \cite{DBLP:conf/acl/YoshikawaST17} & ja & Silver & Yes \\
 &  & \cite{DBLP:conf/naacl/RajendranKCR16} & de, fr & Silver & Yes \\
 &  & \cite{DBLP:conf/acl/HitschlerSR16} & de & Gold & Yes \\
 &  & \cite{DBLP:conf/wmt/ElliottFBBS17} & de, fr & Gold test & Yes \\
 & Visual Genome & \cite{parida-etal-2021-nlphuts} & hi & Gold & Yes \\
 & CC & \cite{caglayan-etal-2021-cross} & de & Silver & Yes \\
 \hline
Transcription & Video Interviews & \cite{jones-muftic-2020-endangered} & kqz, naq & Direct & No \\
 & TED Talks & \cite{karakanta-etal-2020-must} & de, es, fr, it,  &  &  \\
  &  &  & nl, pt, ro & Direct & No \\
 & Wilderness & \cite{DBLP:conf/icassp/Black19} & 700 languages & Direct & Yes (Silver) \\
 & Twitch.tv & \cite{fu-etal-2017-video} & zh-tw, en & Direct & No \\
\hline
Description & IKEA website & \cite{zhou-etal-2018-visual} & en, de, fr & Direct & Close \\
 & Euronews & \cite{afli-etal-2017-multinews} & en, fr, ar, de, es,  &  &  \\
 &  &  & it, pt, tr, ua & Direct & Yes (Silver) \\
\hline
VQA & ImageNet+MSCOCO & \cite{ramnath-etal-2021-worldly} & hi, te & Silver & Yes \\
 &  & \cite{DBLP:conf/nips/GaoMZHWX15} & zh & Gold & No \\
 &  & \cite{koeva-2021-multilingual} & bg, hr, da, nl, en,  & &  \\
 &  &  & fi, fr, el, it, lt, &  &  \\
 &  &  & pl, pt, ro, sk, sl,  &  &  \\
 &  &  & es, sv, sq, is, he, sr & Silver & Yes \\
 & VQA 2.0 & \cite{raj-khan-etal-2021-towards-developing} & hi, bn, es, de, fr, & & \\
  & & & en-hi, en-bn, en-es,  &  &  \\
  & & & en-de, en-fr & Silver & Yes \\
 &  & \cite{gupta-etal-2020-unified} & hi, en-hi & Silver & Yes \\
 & Visual Genome & \cite{shimizu-etal-2018-visual} & ja & Gold & Yes (Subset) \\
\hline
Dialog & Matterport3D & \cite{ku-etal-2020-room} & hi, te & Gold & No \\
 & Pentomino puzzle & \cite{zarriess-etal-2016-pentoref} & en, de & Gold & Yes \\
\hline
Comparison &  & \cite{liu-etal-2021-visually} & id, zh, sw, ta, tr & Gold & No \\
\hline
Misc &  & \cite{alberts-etal-2021-visualsem} & ar, zh, nl, en,  &  &  \\
 &  &  & fa, fr, de, it,  &  &  \\
 &  &  & ko, pl, pt, ru, &  &  \\
 &  &  & es, sv & Silver & Yes \\
 &  & \cite{moneglia-etal-2014-imagact} & it, zh, es & Silver + Gold & No \\
 &  & \cite{gella-etal-2019-cross} & de, es & Silver + Gold & Yes \\
Sentiment Recogn. & Youtube monologues & \cite{bagher-zadeh-etal-2020-cmu} & es, pt, de, fr & Gold & No \\
\hline
\end{tabular}
}
\caption{\small Datasets along with languages (ISO codes) spanned, gold/silver nature of annotations and parallism across languages.}
\label{tab:datasets}
\end{table*}

%%%%%%%%%%%% end

==> tables/models.tex <==
%%%%%%%%%%%%%%%% start

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[tbh]
\centering
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{llllll}
\hline
\textbf{Modeling} &  &  &  &  &  \\
\textbf{Category} & \textbf{Sub-category} & \textbf{Work} & \textbf{Cross-lingual?} & \textbf{AV Features} & \textbf{Text Features} \\
\hline
Modular & Translation-first & \cite{arora-etal-2020-investigative} & No & MFCC (speech) & Phrase \\
 &  & \cite{route-etal-2019-multimodal} & No & MFCC (speech) & LSTM \\
 &  & \cite{ramnath-etal-2021-worldly} & Yes & MFCC (speech) & LSTM \\
 &  & \cite{de-melo-weikum-2010-providing} & Yes & - & Surface forms \\
 & Additional data & \cite{gupta-etal-2021-vita} & Yes & Faster R-CNN & mBART \\
 &  & \cite{lala-etal-2018-sheffield} & Yes & ResNet-50 & MUSE \\
 &  & \cite{calixto-liu-2017-incorporating} & Yes & VGG-19 & RNN \\
 \hline
Embedding & Fusion & \cite{DBLP:conf/iclr/0001C0USLZ20} & No & ResNet-50 & Transformer \\
Projection &  & \cite{parida-etal-2021-nlphuts} & Yes & CNN & LSTM \\
 &  & \cite{caglayan-etal-2021-cross} & Yes & Faster R-CNN & Transformer \\
 &  & \cite{parida-etal-2020-odianlps} & Yes & InceptionResNetv2 & Transformer \\
 &  & \cite{gella-etal-2019-cross} & Yes & ResNet-34 & Word2Vec \\
 &  & \cite{fu-etal-2017-video} & No & ResNet34-LSTM & Char-LSTM \\
 & Multiplication & \cite{susanto-etal-2021-rakutens} & Yes & UVR & mBART \\
 &  & \cite{fei-etal-2021-cross} & No & CLIP image encoder & CLIP text encoder(English)+SBERT \\
 &  &  &  & & paraphrase-multilingualmpnet-base-v2 \\
 &  &  &  & & (for other languages) \\
 &  & \cite{ku-etal-2020-room} & Yes & EfficientNetB4 CNN & mBERT \\
 &  & \cite{shi-etal-2019-visually} & No & ResNet-101 & FastText \\
 &  & \cite{mohammadshahi-etal-2019-aligning-multilingual} & Yes & ResNet-152 & FastText \\
 & CCA & \cite{nakayama-etal-2020-visually} & Yes & Faster-RCNN, VGG16, & MeCab tokenizer, \\
 &  & & & ResNet50 & word vectors \\
 &  & \cite{rotman-etal-2018-bridging} & Yes & VGG-19 & Skip-gram \\
 & Distillation & \cite{raj-khan-etal-2021-towards-developing} & Yes & LXMERT & mBERT \\
\hline
Mapping & Pivot on image & \cite{huang-etal-2021-multilingual} & Yes & R(2+1) spatio-temporal & mBERT \\
 &  &  &  & CNN &  \\
 &  & \cite{huang-etal-2020-unsupervised-multimodal} & Yes & Faster-RCNN & XLM \\
 &  & \cite{kadar-etal-2018-lessons} & Yes & ResNet50 & GRU \\
 &  & \cite{gella-etal-2017-image} & Yes & VGG-19 & GRU \\
 &  & \cite{calixto-liu-2017-sentence} & Yes & VGG-19 & GRU \\
 & Alignment & \cite{fei-etal-2021-cross} & Yes & VL-BERT & VL-BERT \\
 &  & \cite{nishihara-etal-2020-supervised} & Yes & ResNet-50 & Kytea for segmentation \\
 &  & \cite{huang-etal-2019-multi} & Yes & Faster-RCNN & mBERT \\
 & Attention & \cite{ramnath-etal-2021-worldly} & No & Faster R-CNN & IaK \\
 &  & \cite{singh-etal-2021-multiple} & Yes & CNN & RNN \\
 &  & \cite{mitzalis-etal-2021-bertgen} & Yes & VL-BERT & mBERT \\
 &  & \cite{imankulova-etal-2020-towards} & Yes & ResNet-50 & RNN \\
 &  & \cite{bagher-zadeh-etal-2020-cmu} & No & Conv1D + Transformer & Conv1D + Transformer \\
 &  & \cite{gupta-etal-2020-unified} & Yes & R-CNN & fastText, CNN \\
 &  & \cite{zhou-etal-2018-visual} & Yes & ResNet & LSTM \\
 &  & \cite{shimizu-etal-2018-visual} & Yes & VGG-19 & LSTM \\
\hline
Other &  & \cite{karakanta-etal-2021-simultaneous} & No & CNN & CNN \\
 &  & \cite{liu-etal-2021-visually} & No & baselines & baselines \\
 &  & \cite{karakanta-etal-2020-must} & Yes & No images just NMT & Transformer \\
 &  & \cite{vilares-etal-2020-bringing} & No & X, Y coordinates & (linguistic ftrs) \\
 \hline
\end{tabular}
}
\caption{\small Categories of modeling approaches serving cross-lingually with feature representations for modalities and languages.}
\label{tab:methods}
\end{table*}


%%%%%%%%%%%%%%%% end
